Evaluating computational models of infant phonetic learning across languages

In the first year of life, infants' speech perception becomes attuned to the sounds of their native language. Many accounts of this early phonetic learning exist, but computational models predicting the attunement patterns observed in infants from the speech input they hear have been lacking. A recent study presented the first such model, drawing on algorithms proposed for unsupervised learning from naturalistic speech, and tested it on a single phone contrast. Here we study five such algorithms, selected for their potential cognitive relevance. We simulate phonetic learning with each algorithm and perform tests on three phone contrasts from different languages, comparing the results to infants' discrimination patterns. The five models display varying degrees of agreement with empirical observations, showing that our approach can help decide between candidate mechanisms for early phonetic learning, and providing insight into which aspects of the models are critical for capturing infants' perceptual development.

==> background.tex <==
\section{Background}

\citet{schatz2019} presented the first computational model of early phonetic learning from unsegmented speech data. They trained the model on either American English or Japanese speech and tested its ability to discriminate the American English [\textipa{\*r}]--[l] contrast depending on the training language. The `native' model (trained on American English) showed significantly higher discrimination scores than the `non-native' model (trained on Japanese), without acquiring explicit categorical representations.
This suggests that phonetic categories may not be the only type of representations compatible with the existing discrimination data. At the same time, phone discrimination results from infants are available for a large variety of phonetic contrasts and languages, and the proposed account of representation learning needs to be tested on them. Moreover, \citeauthor{schatz2019}'s model is just one implementation of the distributional learning account without phonetic categories: many models in the field of speech processing implement this general idea under very different assumptions.

Here, we focus on the results of three behavioral experiments with infants, motivated by (1) the availability of corresponding speech corpora for training computational models, and (2) the robustness of the empirical results in the literature:
\begin{enumerate}[topsep=0pt, itemsep=-5pt]
    \item \citet{kuhl2006}, with American English and Japanese infants tested on the English [\textipa{\*r}]--[l] contrast. In a conditioned head turn procedure, English- and Japanese-learning infants showed similar discrimination rates for [\textipa{\*r}a]--[la] at the age of 6--8 months, but English-learning infants showed higher rates at the age of 10--12 months. Similar findings are reported in \citet{tsushima1994}.
    \item \citet{tsao2006}, with Mandarin Chinese and American English infants tested on the Mandarin [\textipa{C}]--[\textipa{\texttctclig \super h}] contrast. Again, conditioned head turn was used: Mandarin- and English-learning infants showed similar discrimination rates for [\textipa{C}i]--[\textipa{\texttctclig \super h}i] at the age of 6--8 months, but Mandarin-learning infants were better at 10--12 months. This is also consistent with the results reported by \citet{kuhl2003}.
    \item \citet{bosch2003}, with Catalan- and Spanish-learning infants tested on the Catalan [e]--[\textipa{E}] contrast. A familiarization-preference procedure was used: at the age of 4 months both groups could discriminate between pseudowords [de\textipa{D}i] and [d\textipa{ED}i], but at 8 months only the Catalan group showed successful discrimination. Consistent results are reported by \citet{albareda2011}, who used anticipatory eye movements.
\end{enumerate}

We consider five different models of representation learning (see Table~\ref{tbl:models}), varying in terms of (1) learning mechanisms: bottom-up (building up representations from frame-level segments) vs.\ top-down (using longer sound sequences to learn something about their `atomic' representations), (2) presence of supervision: fully unsupervised vs.\ weakly supervised models, and (3) dealing with the time dimension: preserving the sequential structure of the acoustic segments vs. encoding sequences into vectors with fixed dimensionality. The details of each model are provided in the next section.

